Self-Supervised Learning based CT Denoising using Pseudo-CT Image Pairs

Recently, Self-supervised learning methods able to perform image denoising without ground truth labels have been proposed. These methods create low-quality images by adding random or Gaussian noise to images and then train a model for denoising. Ideally, it would be beneficial if one can generate high-quality CT images with only a few training samples via self-supervision. However, the performance of CT denoising is generally limited due to the complexity of CT noise. To address this problem, we propose a novel self-supervised learning-based CT denoising method. In particular, we train pre-train CT denoising and noise models that can predict CT noise from Low-dose CT (LDCT) using available LDCT and Normal-dose CT (NDCT) pairs. For a given test LDCT, we generate Pseudo-LDCT and NDCT pairs using the pre-trained denoising and noise models and then update the parameters of the denoising model using these pairs to remove noise in the test LDCT. To make realistic Pseudo LDCT, we train multiple noise models from individual images and generate the noise using the ensemble of noise models. We evaluate our method on the 2016 AAPM Low-Dose CT Grand Challenge dataset. The proposed ensemble noise model can generate realistic CT noise, and thus our method significantly improves the denoising performance existing denoising models trained by supervised- and self-supervised learning.

==> files/introduction_relatedwork.tex <==
\section{Introduction}

Computed Tomography (CT) imaging is one of the most widely used non-invasive imaging techniques for diagnosis, stage classification and disease detection. However, even with high availability, radiation from CT scans can potentially harm patients []. Accordingly, low-dose CT (LDCT) scanners are being developed to reduce the potential radiation damage to patients, but the LDCT images often contain noises and thus cause inaccurate diagnosis. To address this problem, machine learning [] and deep learning [] techniques have been proposed to make high quality images by denoising the LDCT images. 

Although the deep learning methods have improved the denoising performance significantly by learning dense model parameters to minimize the difference between LDCT and normal-dose CT (NDCT), spatial redundancy between feature maps is not alleviated during training, and thus many parameters are used for processing low frequency signals with high redanduncy. Thus, it is difficult to properly handle the high frequency signals that are important for CT denoising. Figure 1 shows an evidence of the importance of learning high frequency components for denoising. Most of the residuals between low- and normal-dose CTs are located in the high frequency band in frequency domain. Thus, in general, the traditional deep learning methods for image quality improvement often generate over-smoothed images, making it difficult to distinguish the detailed structures.

To address this problem, we propose a novel CT denoising method that divides an image into low and high frequency components and learns the parameters more focusing on the high frequency information. We introduce a novel CT denoising network consisting of octave convolution which takes in feature maps with two frequencies and extracts information directly from the low-frequency maps without the need of decoding it back to the high-frequency. We extend the octave convolution and integrate this convolution on the residual network to effectively reduce the spatial redanduncy. Furthermore, we optimize this network with a novel edge loss with L1 and perceptual losses to maintain the detailed edges and styles while suppressing noises.

The main contributions of this work are as follow: (1) We adopt multi-scare representation learning to the CT denoising problem. Spatial redundancy in low frequency components is implicitly alleviated in our network. (2) We extend the 2D octave convolution proposed in image classification to image denoising problem. Since there are lots of spatial redundancy in 2D space, the characteristics of octave convolution are the most suitable for the CT denoising. We empirically show the benefit of octave convolution applied to CT denoising. (3) Lastly, we integrate a novel edge loss function and use it with L1 and perceptual losses in order to suppress the noise while remaining the edge sharpness. The proposed method can be applied to not only denoising but also various medical image quality enhancement problems.

\subsection{Related work}
\noindent{\textbf{CT denoising:}} For LDCT denoising, several techniques such as non-local means [XX], dictionary learning [XX], and black matching [XX] have been proposed. These methods perform the denoising using relevant dictionary patches searched from a target image or from training images. Model-based iterative reconstruction (MBIR) methods [] also have been studied to further impose additional requirements such as smoothness or sparsity. Though these methods generated reasonable denoising results, the performance was often limited due to the non-uniform distribution of LDCT noise. 

Recently, deep learning based methods have been proposed. For example, Chen et al. [1] first proposed a convolutional neural network (CNN) consisting of 3 convolutional layers to minimize the mean square error (MSE) between the prediction and NDCT. Yang et al. [6] proposed a deeper network with the perceptual loss to preserve structural details. Chen et al. [9] proposed an encoder-decoder network with residual paths, while Yang et al. [7] proposed a ResNet. M. Gholizadeh-Ansari et al. [3] proposed a dilated residual network to capture contextual information of a large receptive field and used a non-trainable edge detector to utilize the edge of LDCT for learning. However, above-mentioned approaches cannot capture low and high-frequency feature representations separately in the process of feature embedding. In image reconstruction network, mixed feature representation cannot accurately guide the generation of high-frequency and low-frequency regions, which is not conducive to restoring details and maintaining structural similarity. 

Recently, Kang et al. [8] proposed a method that performs a wavelet transform to divide an image into different frequency components and then learn a CNN to minimize the difference between these components with the frequency components of a denoised image. This method is most relevant to the proposed method in that it learns a network for processing in the frequency domain by decomposing the image into different components. However, this method does not provide a way to reduce the spatial redundancy; \textit{i.e.}, it performs the wavelet transform explicitly and then learns the network using all these coefficients with concatenation. The proposed method performs the decomposition within the network and effectively reduces the spatial redundancy.

% to reduce the noise while precisely preserving the structure of CT images

\noindent{\textbf{Multi-scale Representation Learning:}} Several studies have been conducted to decompose a signal or an image into multiple scales and then process them. Dai et al. [17] decomposed EEG signals into different frequency bands, extracted features using CNN, and then performed classification using the concatenate features. Chen et al. [16] transformed the input data into different scales, and performed object and speech recognition using the features obtained from several scales. [25] proposed the MG-Conv operator to represent a multi-grid pyramid feature representation for image classification. Chen et al. [2] proposed the octave convolution to separate low- and high-frequency features effectively reduce the spatial redundancy of low frequency components. Inspired by this concept applied to the classification tasks, the proposed method performs the multi-scale learning for the CT denoising. To do so, we integrate octave convolution into the proposed denoising network that learns residuals between LDCT and NDCT.
